Evaluating Gender Bias in Machine Translation

We present the first challenge set and evaluation protocol for the analysis of gender bias in machine translation (MT). Our approach uses two recent coreference resolution datasets composed of English sentences which cast participants into non-stereotypical gender roles (e.g., "The doctor asked the nurse to help her in the operation"). We devise an automatic gender bias evaluation method for eight target languages with grammatical gender, based on morphological analysis (e.g., the use of female inflection for the word "doctor"). Our analyses show that four popular industrial MT systems and two recent state-of-the-art academic MT models are significantly prone to gender-biased translation errors for all tested target languages. Our data and code are made publicly available.

==> background.tex <==
%% \begin{itemize}
%% \item Biases in coreference.
%% \item Recent popular publications identify anecdotal evidence to gender bias in NMT. Google also implemented
%%   a feature to manually control for gender in translation.
%% \item Little work in quantitative analysis to back this, and to measure the extent to which current state-of-the-art systems are prone to
%%   exhibit such biases.
%% \item Most relevant to our work, \cite{Prates2018AssessingGB}, ...
%% \end{itemize}

%% \luke{I am a little confused about this section. The fist (and second) paragraphs are related work, while second and third introduce new ideas for the data methods. Maybe consider merging related work into intro (or separate bvery short section) and make a section here about data?}

% Interest in bias in ML in general: vision, social, etc.
%Recently, there has been a rising awareness of the ways in which social biases in training data affect machine learning models. % \nascomment{through training data?}.

%% For example, in the sentence at the top of Figure \ref{fig:flow}, a biased
%% system might make the stereotypical prediction to link the pronoun ``he''
%% with ``manager'',
%% while native English speakers can easily make the less common association
%% between the masculine pronoun and ``cleaner'', based solely on the context of the
%% sentence.
%% While both Winogender and Winobias are balanced between gender and professions
%% (e.g., for every example there is a counter example where gender are flipped),
%% \newcite{\coref} have shown that state-of-the-art coreference resolution systems
%% are indeed prone to echo gender biases in their training data, resorting to it
%% when making their predictions, rather than relying on the context in the sentences.

In recent years, several challenge sets were created in order to evaluate MT accuracy on particular tasks, such as
argument switching or subjunctive moods \cite{Isabelle2017ACS}, discourse phenomena \cite{Bawden2018EvaluatingDP}, or correct pronoun translation \cite{DBLP:journals/corr/abs-1810-02268}.

In this work we create a challenge set for gender bias in MT (which we dub ``\ds'') via a simple deterministic conversion
of the \wg\ and \wb\ coreference test sets to associate between entities and their gender.
Where the original corpora have coreference links between pronouns and entities (e.g., ``her'' and ``doctor'' in Figure 1),
\ds\ would have a gender (``female'') associated with the entity.
Specifically, each instance in \ds\ is composed of the following three elements: %\nascomment{slightly unclear:  what do the two existing datasets offer and what had to be done to create this dataset?  some readers might think there was some automatic NLP applied, or more annotation.  I think it was purely a deterministic and simple join ... but we should say so}
%\begin{enumerate}
(1) An English sentence which follows the Winograd schema, as shown in Figure \ref{fig:flow}.
(2) A target entity within the sentence (e.g, ``the doctor'').
(3) The gender of the entity: either ``male'', ``female'', or ``neutral'' (in case
the gender is ambiguous), which we automatically identify by the referring pronoun.
%\end{enumerate}

Overall, \ds\ contains 3,888 instances, and is equally balanced between male and female genders, as well as between stereotypical and non-stereotypical gender-role assignments
(e.g., a female doctor versus a female nurse).
Additional dataset statistics are presented in Table \ref{tab:dataset}.

In the following sections we will use MT models to
translate the input sentence to languages with grammatical gender,
and automatically extract the gender of the input entity in the \emph{target} language,
which we can then compare with the gold English gender.

\input{tables/dataset}

%\nascomment{The figure is a good start; I would suggest annotating it more and contrasting a good example with a bad one.}

